EGOSTREAM: A Diagnostic Benchmark for Streaming Episodic Memory in Egocentric Vision

Continuous episodic memory is a core capability for autonomous agents operating in dynamic, real-world environments, yet current streaming video benchmarks provide limited tools for diagnosing what models remember and for how long. We introduce EGOSTREAM, a diagnostic benchmark for streaming episodic memory evaluation in egocentric vision. EGOSTREAM organizes 2,250 curated questions along seven cognitive dimensions: detail, spatial, temporal, event, social, causal, and prospective memory. We introduce the Answer Validity Window (AVW), which specifies the temporal span an answer remains valid as the observed scene evolves. This allows us to expand the questions into 8,528 recall-conditioned evaluations, enabling controlled testing from instant to ultra-long-term recall while separating genuine model forgetting from natural world-state changes. We rigorously establish baseline performance through a unified streaming MLLM framework that compares several state-of-the-art memory-management mechanisms, covering sliding windows, attention sinks, KV-cache pruning, merging, adaptive head budgets, and offloading. Experiments on a unified Qwen3-VL backbone, with consistent trends on Molmo2-8B and InternVL3.5-8B, reveal that comparable aggregate accuracies mask starkly different memory profiles. For instance, token pruning preserves fine-grained details and temporal structure significantly better than token merging, adaptive head budgets yield the highest aggregate semantic accuracy, while quantized offloading rescues ultra-long-term recall. Ultimately, all in-cache memory policies operate well below real-time (>1s per frame), and top performing in-cache methods ceil at about 45% accuracy under a 9,804-token budget, exposing critical gaps in current architectures. EGOSTREAM provides the diagnostic testbed needed to close these gaps. Project website: https://coai-iplab.github.io/EgoStream/

==> Tables/controlled_results_table.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}

\caption{\textbf{Controlled Diagnostic Evaluation.}
Comparison of memory-management strategies under the same MLLM setting.
Badges summarize the active cache policy. Accuracy is reported globally, by semantic category,
and by temporal recall regime.}
\label{tab:controlled_results}

\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}r p{4.5cm} c c ccccccc ccccccc@{}}
\toprule
\textbf{\#} &
\textbf{Policy} &
\textbf{Acc} &
\textbf{Avg Acc} &
\multicolumn{7}{c}{\textbf{Semantic Categories}} &
\multicolumn{7}{c}{\textbf{Temporal Recall Regimes}} \\
\cmidrule(lr){5-11}
\cmidrule(l){12-18}
&&&
& \textbf{SPAT}
& \textbf{TEMP}
& \textbf{DETL}
& \textbf{EVNT}
& \textbf{SOC}
& \textbf{CAUS}
& \textbf{PROS}
& \textbf{Inst}
& \textbf{Short}
& \textbf{S-Mid}
& \textbf{Mid}
& \textbf{M-Long}
& \textbf{Long}
& \textbf{Ultra} \\
\midrule

\multicolumn{18}{@{}l}{\textit{Sliding-window baselines}} \\

17 & \bSW
   & 30.3 & 30.3 & 30.7 & 34.2 & 31.0 & 30.7 & 27.9 & 25.3 & 31.9 & 32.1 & 31.3 & 29.8 & 28.4 & 29.0 & 28.7 & 27.6 \\

1 & \bSW\ \bSink
   & 47.1 & 44.7 & 57.9 & 51.2 & 54.9 & 46.4 & 28.9 & 38.7 & 35.2 & 55.1 & 55.1 & 49.2 & 40.0 & 29.3 & 24.9 & 19.7 \\

2 & \bSW\ \bSink\ \bHat
   & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

\midrule
\multicolumn{18}{@{}l}{\textit{Similarity-based compression} \bSink\ \bHat} \\

3 & + \bMerge
   & 52.4 & 53.0 & 54.4 & 50.5 & 57.9 & 47.3 & 58.8 & 38.4 & 63.4 & 58.2 & 56.1 & 51.7 & 44.7 & 37.1 & 25.0 & -- \\

20 & + \bMerge\ \bIntraCos
   & 46.0 & 43.4 & 57.3 & 49.8 & 53.3 & 45.9 & 27.5 & 38.5 & 31.6 & 54.4 & 53.2 & 48.2 & 39.4 & 27.5 & 22.9 & 21.1 \\

21 & + \bMerge\ \bIntraPA
   & 44.2 & 41.9 & 54.3 & 48.2 & 51.5 & 42.5 & 28.3 & 37.5 & 30.9 & 52.5 & 52.0 & 44.0 & 37.2 & 28.7 & 23.5 & 26.3 \\

23 & + \bMerge\ \bIntraPA\ \bPrune\ \bInterPA
   & 50.8 & 47.7 & 57.2 & 56.1 & 56.1 & 47.4 & 30.9 & 40.2 & 46.2 & 57.6 & 56.2 & 51.2 & 43.6 & 31.0 & 26.6 & -- \\

4 & + \bPrune
   & 56.1 & 55.4 & 57.2 & 58.0 & 61.8 & 50.8 & 62.3 & 40.0 & 57.7 & 61.1 & 61.1 & 55.4 & 47.7 & 41.8 & 0.0 & -- \\

5 & + \bPrune\ \bIntraCos
   & 48.1 & 45.6 & 60.5 & 52.4 & 56.6 & 46.6 & 28.5 & 39.9 & 34.9 & 55.6 & 55.0 & 52.2 & 41.3 & 30.6 & 24.9 & 15.8 \\

6 & + \bPrune\ \bIntraPA
   & 47.8 & 45.1 & 59.5 & 53.1 & 56.5 & 45.9 & 28.7 & 39.3 & 32.9 & 56.0 & 54.7 & 50.2 & 40.6 & 30.8 & 22.6 & 35.5 \\

7 & + \bPrune\ \bIntraCS
   & 45.4 & 43.1 & 51.9 & 52.4 & 52.6 & 43.9 & 27.3 & 38.2 & 35.5 & 52.6 & 50.4 & 46.5 & 39.5 & 28.5 & 26.9 & 30.2 \\

8 & + \bPrune\ \bIntraVN
   & 46.3 & 43.9 & 56.4 & 54.4 & 54.3 & 44.2 & 27.5 & 39.6 & 30.9 & 54.0 & 51.9 & 48.1 & 42.1 & 28.6 & 25.2 & 25.7 \\

9 & + \bPrune\ \bInterPA
   & 47.7 & 45.4 & 59.9 & 55.5 & 56.2 & 45.7 & 27.3 & 38.5 & 34.9 & 55.4 & 54.3 & 49.4 & 42.8 & 30.8 & 24.3 & 25.0 \\

10 & + \bPrune\ \bInterCos
   & 47.4 & 45.2 & 57.9 & 53.8 & 55.6 & 45.8 & 28.0 & 39.7 & 35.9 & 54.7 & 52.8 & 48.8 & 43.9 & 30.8 & 26.4 & 23.7 \\

11 & + \bPrune\ \bIntraVN\ \bInterCos
   & 47.3 & 44.7 & 58.2 & 55.3 & 55.6 & 45.5 & 27.5 & 39.9 & 31.2 & 54.4 & 53.8 & 49.5 & 42.8 & 32.1 & 18.8 & 19.4 \\

12 & + \bPrune\ \bIntraPA\ \bInterPA
   & 49.6 & 46.6 & 59.4 & 57.0 & 57.7 & 46.7 & 28.9 & 41.6 & 34.8 & 57.3 & 56.0 & 51.8 & 42.8 & 30.4 & 24.3 & 23.4 \\

13 & + \bPrune\ \bIntraVN\ \bInterPA
   & 48.4 & 45.5 & 58.3 & 56.3 & 57.1 & 46.4 & 25.7 & 42.9 & 32.0 & 56.0 & 53.9 & 50.1 & 43.2 & 32.3 & 24.7 & 23.3 \\

14 & + \bPrune\ \bIntraCS\ \bInterPA
   & 48.5 & 45.6 & 57.5 & 54.0 & 56.3 & 46.9 & 28.1 & 41.6 & 34.6 & 56.4 & 55.7 & 49.4 & 40.8 & 31.1 & 24.1 & 25.0 \\

15 & + \bPrune\ \bIntraVN\ \bInterCos
   & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

16 & + \bPrune\ \bIntraPA\ \bInterCos
   & 49.8 & 46.4 & 58.0 & 57.5 & 58.6 & 48.0 & 28.5 & 40.2 & 34.2 & 56.3 & 56.2 & 52.7 & 43.4 & 32.2 & 22.7 & 21.7 \\

\midrule
\multicolumn{18}{@{}l}{\textit{Offloading-based memory management} \bSW \bSink\ \bHat} \\

18 & + \bOff
   & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

19 & + \bOff\ \bQOff
   & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\

\bottomrule
\end{tabular}%
}

\vspace{3pt}
\footnotesize
\textbf{Badge legend.}
\bSW\ Sliding Window;
\bSink\ Sink tokens;
\bHat\ Hat tokens;
\bMerge\ Similarity merging;
\bPrune\ Similarity pruning;
\bIntraPA\ Intra-frame pseudo-attention;
\bInterPA\ Inter-frame pseudo-attention;
\bIntraCos\ Intra-frame cosine;
\bInterCos\ Inter-frame cosine;
\bIntraCS\ Intra-frame cross-sink;
\bIntraVN\ Intra-frame value norm;
\bOff\ disk offloading;
\bQOff\ quantized offloading.

\end{table*}


==> Tables/controlled_results_table_heatmap.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Controlled evaluation of memory-management strategies.} Accuracy is reported across semantic categories and temporal recall regimes, alongside per-frame processing time. Applicable configurations are mapped to their closest equivalent in literature wrt isolated memory strategies.}
\label{tab:controlled_eval}
\ifcsname c@rowcount\endcsname\else\newcounter{rowcount}\fi
\setcounter{rowcount}{0}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}r p{5cm} c c c c c c c c c c c c c c c c c c@{}}
\toprule
 &  &  & \multicolumn{8}{c}{\textbf{Semantic Categories}} & \multicolumn{8}{c}{\textbf{Temporal Recall Regimes}} & \multicolumn{1}{c}{\textbf{Proc.}} \\
\cmidrule(lr){4-11}
\cmidrule(lr){12-19}
%\cmidrule(l){20-20}
 & \textbf{Strategy} & \textbf{Configuration} & \textbf{Avg} & \textbf{SPAT} & \textbf{TEMP} & \textbf{DETL} & \textbf{EVNT} & \textbf{SOC} & \textbf{CAUS} & \textbf{PROS} & \textbf{Avg} & \textbf{Inst} & \textbf{Short} & \textbf{S-Mid} & \textbf{Mid} & \textbf{ML} & \textbf{Long} & \textbf{Ultra} & \textbf{(s)} \\
\midrule
\multicolumn{20}{@{}l}{\textit{Sliding-window baselines}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_sw_pura} & \bFIFO & Sliding Window & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{29.53} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.50} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{33.53} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.62} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.02} & \cellcolor[HTML]{D5EFCF}\textcolor[HTML]{000000}{26.85} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{25.94} & \cellcolor[HTML]{D3EECD}\textcolor[HTML]{000000}{29.28} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{28.33} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{31.83} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{31.09} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{28.71} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.80} & \cellcolor[HTML]{CBEAC4}\textcolor[HTML]{000000}{28.42} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{28.12} & \cellcolor[HTML]{AEDEA7}\textcolor[HTML]{000000}{22.37} & \cellcolor[HTML]{FFF5F0}\textcolor[HTML]{000000}{1.05} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sw_sink}\label{row:q3vl8b_sw_sink_aaaaa} & \bFIFO\ \bSink & StreamVLM~\cite{xu2025streamingvlm} & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{44.74} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{57.95} & \cellcolor[HTML]{248C46}\textcolor[HTML]{FFFFFF}{51.22} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{54.90} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{46.36} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{28.87} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{38.68} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{35.20} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{39.05} & \cellcolor[HTML]{005120}\textcolor[HTML]{FFFFFF}{55.06} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{55.10} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{49.18} & \cellcolor[HTML]{208843}\textcolor[HTML]{FFFFFF}{40.00} & \cellcolor[HTML]{7FC97F}\textcolor[HTML]{000000}{29.34} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{24.93} & \cellcolor[HTML]{D3EECD}\textcolor[HTML]{000000}{19.74} & \cellcolor[HTML]{FFF4EF}\textcolor[HTML]{000000}{1.07} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based merge \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_pseudo_att} & \bMerge\ \bIntraPA & CaM-like~\cite{zhang2024cam} & \cellcolor[HTML]{1E8741}\textcolor[HTML]{FFFFFF}{41.87} & \cellcolor[HTML]{17813D}\textcolor[HTML]{FFFFFF}{54.25} & \cellcolor[HTML]{43AC5E}\textcolor[HTML]{FFFFFF}{48.20} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{51.49} & \cellcolor[HTML]{248C46}\textcolor[HTML]{FFFFFF}{42.48} & \cellcolor[HTML]{5DB96B}\textcolor[HTML]{FFFFFF}{28.27} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{37.48} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{30.92} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{37.73} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{52.47} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{51.98} & \cellcolor[HTML]{3BA458}\textcolor[HTML]{FFFFFF}{44.00} & \cellcolor[HTML]{52B365}\textcolor[HTML]{FFFFFF}{37.20} & \cellcolor[HTML]{BAE3B3}\textcolor[HTML]{000000}{28.65} & \cellcolor[HTML]{B7E2B1}\textcolor[HTML]{000000}{23.48} & \cellcolor[HTML]{66BD6F}\textcolor[HTML]{000000}{26.32} & \cellcolor[HTML]{FC8B6B}\textcolor[HTML]{000000}{2.87} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_cosine} & \bMerge\ \bIntraCos & CaM-like~\cite{zhang2024cam} & \cellcolor[HTML]{03702E}\textcolor[HTML]{FFFFFF}{43.42} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{57.30} & \cellcolor[HTML]{329B51}\textcolor[HTML]{FFFFFF}{49.83} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{53.28} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{45.87} & \cellcolor[HTML]{A4DA9E}\textcolor[HTML]{000000}{27.52} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{38.53} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{258D47}\textcolor[HTML]{FFFFFF}{38.10} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{54.44} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{53.20} & \cellcolor[HTML]{0C7735}\textcolor[HTML]{FFFFFF}{48.18} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{39.40} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.50} & \cellcolor[HTML]{CFECC9}\textcolor[HTML]{000000}{22.90} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{FCB296}\textcolor[HTML]{000000}{2.33} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based hybrid merge + prune \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_pseudo_att_inter_pseudo_att} & \bMerge\ \bIntraPA\ \bPrune\ \bInterPA & -- & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{43.44} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{56.66} & \cellcolor[HTML]{147E3A}\textcolor[HTML]{FFFFFF}{52.62} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{53.89} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{45.33} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{26.10} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{38.23} & \cellcolor[HTML]{8ACE88}\textcolor[HTML]{000000}{31.25} & \cellcolor[HTML]{268E47}\textcolor[HTML]{FFFFFF}{38.01} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{54.61} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{52.87} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{47.35} & \cellcolor[HTML]{228A44}\textcolor[HTML]{FFFFFF}{39.87} & \cellcolor[HTML]{A8DCA2}\textcolor[HTML]{000000}{28.88} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{21.45} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{8A0812}\textcolor[HTML]{FFFFFF}{5.32} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based prune \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cross_sink} & \bPrune\ \bIntraCS & StreamMem~\cite{yang2025streammem} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{42.39} & \cellcolor[HTML]{29914A}\textcolor[HTML]{FFFFFF}{52.25} & \cellcolor[HTML]{1D8640}\textcolor[HTML]{FFFFFF}{51.80} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{52.10} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{43.85} & \cellcolor[HTML]{BCE4B5}\textcolor[HTML]{000000}{27.23} & \cellcolor[HTML]{03702E}\textcolor[HTML]{FFFFFF}{37.93} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{38.88} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{52.12} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{50.64} & \cellcolor[HTML]{289049}\textcolor[HTML]{FFFFFF}{45.82} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{39.07} & \cellcolor[HTML]{CBEAC4}\textcolor[HTML]{000000}{28.42} & \cellcolor[HTML]{3BA458}\textcolor[HTML]{FFFFFF}{25.80} & \cellcolor[HTML]{278F48}\textcolor[HTML]{FFFFFF}{30.26} & \cellcolor[HTML]{B01217}\textcolor[HTML]{FFFFFF}{4.91} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm} & \bPrune\ \bIntraVN & InfiniPot-V (VaN)~\cite{kim2025infinipotv} & \cellcolor[HTML]{00692A}\textcolor[HTML]{FFFFFF}{43.79} & \cellcolor[HTML]{0B7734}\textcolor[HTML]{FFFFFF}{55.54} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{53.67} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{52.49} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{45.98} & \cellcolor[HTML]{238B45}\textcolor[HTML]{FFFFFF}{29.02} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{38.23} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{39.17} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{54.30} & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{51.87} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{46.88} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{41.93} & \cellcolor[HTML]{9FD899}\textcolor[HTML]{000000}{29.00} & \cellcolor[HTML]{5AB769}\textcolor[HTML]{FFFFFF}{25.22} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{DC2924}\textcolor[HTML]{FFFFFF}{4.23} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_inter_cosine} & \bPrune\ \bInterCos & InfiniPot-V (TaR)~\cite{kim2025infinipotv} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{45.23} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{57.87} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{53.78} & \cellcolor[HTML]{005120}\textcolor[HTML]{FFFFFF}{55.60} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{45.76} & \cellcolor[HTML]{73C476}\textcolor[HTML]{000000}{28.05} & \cellcolor[HTML]{00471C}\textcolor[HTML]{FFFFFF}{39.73} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{35.86} & \cellcolor[HTML]{006529}\textcolor[HTML]{FFFFFF}{40.16} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{54.75} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{52.76} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{48.82} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{43.87} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{258D47}\textcolor[HTML]{FFFFFF}{26.38} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{23.68} & \cellcolor[HTML]{AB1016}\textcolor[HTML]{FFFFFF}{4.99} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm_inter_cosine} & \bPrune\ \bIntraVN\ \bInterCos & InfiniPot-V~\cite{kim2025infinipotv} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{44.52} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{58.91} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{56.23} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{55.51} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{46.36} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{26.10} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{39.58} & \cellcolor[HTML]{DDF2D8}\textcolor[HTML]{000000}{28.95} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{40.22} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{54.44} & \cellcolor[HTML]{005321}\textcolor[HTML]{FFFFFF}{53.93} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{50.12} & \cellcolor[HTML]{006428}\textcolor[HTML]{FFFFFF}{42.27} & \cellcolor[HTML]{268E47}\textcolor[HTML]{FFFFFF}{30.38} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{21.45} & \cellcolor[HTML]{37A055}\textcolor[HTML]{FFFFFF}{28.95} & \cellcolor[HTML]{D11E1F}\textcolor[HTML]{FFFFFF}{4.42} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:0_12_q3vl8b_sim_prune_intra_pseudo_att_inter_cosine_octer} & \bPrune\ \bIntraPA\ \bInterCos & StreamTOM~\cite{chen2025streamingtom} w/o \bOff & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{45.19} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{57.87} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{57.28} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.68} & \cellcolor[HTML]{00471C}\textcolor[HTML]{FFFFFF}{46.58} & \cellcolor[HTML]{55B567}\textcolor[HTML]{FFFFFF}{28.35} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{37.78} & \cellcolor[HTML]{72C375}\textcolor[HTML]{000000}{31.79} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{40.43} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{55.42} & \cellcolor[HTML]{004D1F}\textcolor[HTML]{FFFFFF}{54.37} & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{50.88} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{41.73} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{31.07} & \cellcolor[HTML]{37A055}\textcolor[HTML]{FFFFFF}{25.88} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{23.68} & \cellcolor[HTML]{77040F}\textcolor[HTML]{FFFFFF}{5.51} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cosine} & \bPrune\ \bIntraCos & -- & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{45.63} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{60.51} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{52.39} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.61} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{46.64} & \cellcolor[HTML]{45AD5F}\textcolor[HTML]{FFFFFF}{28.50} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{39.88} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{34.87} & \cellcolor[HTML]{0B7734}\textcolor[HTML]{FFFFFF}{39.34} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{55.60} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{54.99} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{52.18} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{41.27} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{30.61} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{24.93} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{15.79} & \cellcolor[HTML]{FCB69B}\textcolor[HTML]{000000}{2.28} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_pseudo_att} & \bPrune\ \bIntraPA & -- & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{45.12} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{59.47} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{53.08} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{56.52} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{45.87} & \cellcolor[HTML]{359E53}\textcolor[HTML]{FFFFFF}{28.72} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{39.28} & \cellcolor[HTML]{3EA75A}\textcolor[HTML]{FFFFFF}{32.89} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{41.50} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.04} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{54.71} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{50.18} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{40.60} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{DAF0D4}\textcolor[HTML]{000000}{22.61} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{35.53} & \cellcolor[HTML]{FC8F6F}\textcolor[HTML]{000000}{2.82} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_inter_pseudo_attn} & \bPrune\ \bInterPA & -- & \cellcolor[HTML]{00481D}\textcolor[HTML]{FFFFFF}{45.42} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{59.87} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{55.53} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{56.17} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{45.65} & \cellcolor[HTML]{B6E2AF}\textcolor[HTML]{000000}{27.30} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{38.53} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{34.87} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{40.30} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{55.42} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{54.32} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{49.35} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{42.80} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{8BCF89}\textcolor[HTML]{000000}{24.35} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{B61319}\textcolor[HTML]{FFFFFF}{4.82} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_pseudo_att_inter_pseudo_att} & \bPrune\ \bIntraPA\ \bInterPA & -- & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{44.71} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{58.51} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{55.30} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{56.52} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{45.54} & \cellcolor[HTML]{3FA85B}\textcolor[HTML]{FFFFFF}{28.57} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{39.58} & \cellcolor[HTML]{DDF2D8}\textcolor[HTML]{000000}{28.95} & \cellcolor[HTML]{00682A}\textcolor[HTML]{FFFFFF}{40.03} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{55.55} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{53.87} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{50.29} & \cellcolor[HTML]{00692A}\textcolor[HTML]{FFFFFF}{42.00} & \cellcolor[HTML]{75C477}\textcolor[HTML]{000000}{29.46} & \cellcolor[HTML]{19833E}\textcolor[HTML]{FFFFFF}{26.67} & \cellcolor[HTML]{AEDEA7}\textcolor[HTML]{000000}{22.37} & \cellcolor[HTML]{67000D}\textcolor[HTML]{FFFFFF}{5.66} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm_inter_pseudo_att} & \bPrune\ \bIntraVN\ \bInterPA & -- & \cellcolor[HTML]{005C25}\textcolor[HTML]{FFFFFF}{44.42} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{57.62} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{56.46} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{56.21} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{46.75} & \cellcolor[HTML]{D5EFCF}\textcolor[HTML]{000000}{26.85} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{39.43} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.63} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{39.91} & \cellcolor[HTML]{005020}\textcolor[HTML]{FFFFFF}{55.10} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{54.04} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{50.06} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{42.13} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{30.15} & \cellcolor[HTML]{CFECC9}\textcolor[HTML]{000000}{22.90} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{C1161B}\textcolor[HTML]{FFFFFF}{4.67} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cross_sink_inter_pseudo_att} & \bPrune\ \bIntraCS\ \bInterPA & -- & \cellcolor[HTML]{005C25}\textcolor[HTML]{FFFFFF}{44.39} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{56.74} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{52.50} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{55.56} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{45.22} & \cellcolor[HTML]{278F48}\textcolor[HTML]{FFFFFF}{28.95} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{39.88} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{31.91} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{39.60} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{55.24} & \cellcolor[HTML]{004D1F}\textcolor[HTML]{FFFFFF}{54.43} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{48.12} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{40.60} & \cellcolor[HTML]{3CA559}\textcolor[HTML]{FFFFFF}{30.03} & \cellcolor[HTML]{A9DCA3}\textcolor[HTML]{000000}{23.77} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{B31218}\textcolor[HTML]{FFFFFF}{4.87} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Offloading-based memory management \bFIFO \bSink\ \bHat}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_rekv_offloading} & \bOff & ReKV~\cite{di2025rekv} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{40.99} & \cellcolor[HTML]{2E964D}\textcolor[HTML]{FFFFFF}{51.69} & \cellcolor[HTML]{369F54}\textcolor[HTML]{FFFFFF}{49.48} & \cellcolor[HTML]{2E964D}\textcolor[HTML]{FFFFFF}{48.99} & \cellcolor[HTML]{1E8741}\textcolor[HTML]{FFFFFF}{42.86} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{29.99} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{35.98} & \cellcolor[HTML]{F1FAEE}\textcolor[HTML]{000000}{27.96} & \cellcolor[HTML]{3CA559}\textcolor[HTML]{FFFFFF}{36.83} & \cellcolor[HTML]{137D39}\textcolor[HTML]{FFFFFF}{51.36} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{47.97} & \cellcolor[HTML]{3BA458}\textcolor[HTML]{FFFFFF}{44.00} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{38.67} & \cellcolor[HTML]{8ACE88}\textcolor[HTML]{000000}{29.23} & \cellcolor[HTML]{48AE60}\textcolor[HTML]{FFFFFF}{25.51} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{FDC6B0}\textcolor[HTML]{000000}{2.03} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_rekv_offloading_8bit} & \bQOff & ReKV~\cite{di2025rekv} w/ \bQOff & \cellcolor[HTML]{228A44}\textcolor[HTML]{FFFFFF}{41.63} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{51.85} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{50.64} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{50.83} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{43.63} & \cellcolor[HTML]{A4DA9E}\textcolor[HTML]{000000}{27.52} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{35.38} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{17813D}\textcolor[HTML]{FFFFFF}{38.77} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{52.61} & \cellcolor[HTML]{309950}\textcolor[HTML]{FFFFFF}{47.74} & \cellcolor[HTML]{45AD5F}\textcolor[HTML]{FFFFFF}{43.12} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{39.27} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{30.72} & \cellcolor[HTML]{258D47}\textcolor[HTML]{FFFFFF}{26.38} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{31.58} & \cellcolor[HTML]{FEE2D5}\textcolor[HTML]{000000}{1.59} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:streamtom_like} & \bPrune\ \bIntraPA\ \bInterCos\ \bQOff & StreamingTOM~\cite{chen2025streamingtom} & \cellcolor[HTML]{0C7735}\textcolor[HTML]{FFFFFF}{42.86} & \cellcolor[HTML]{1D8640}\textcolor[HTML]{FFFFFF}{53.61} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{52.39} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{51.88} & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{44.51} & \cellcolor[HTML]{7AC77B}\textcolor[HTML]{000000}{27.97} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{37.78} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{31.91} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{39.93} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{54.03} & \cellcolor[HTML]{278F48}\textcolor[HTML]{FFFFFF}{48.69} & \cellcolor[HTML]{2F984F}\textcolor[HTML]{FFFFFF}{45.06} & \cellcolor[HTML]{208843}\textcolor[HTML]{FFFFFF}{40.00} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{31.42} & \cellcolor[HTML]{2F984F}\textcolor[HTML]{FFFFFF}{26.09} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{34.21} & \cellcolor[HTML]{FEE7DC}\textcolor[HTML]{000000}{1.43} \\

\bottomrule
\end{tabular}%
}
\end{table}

==> Tables/final_table_final_final.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Controlled evaluation of memory-management strategies.} Accuracy is reported across semantic categories and temporal recall regimes, alongside per-frame processing time. Applicable configurations are mapped to their closest equivalent in literature wrt isolated memory strategies.}
\label{tab:controlled_eval}
\ifcsname c@rowcount\endcsname\else\newcounter{rowcount}\fi
\setcounter{rowcount}{0}
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}r p{5cm} c c c c c c c c c c c c c c c c c c@{}}
\toprule
 &  &  & \multicolumn{8}{c}{\textbf{Semantic Categories}} & \multicolumn{8}{c}{\textbf{Temporal Recall Regimes}} & \multicolumn{1}{c}{\textbf{Time (s)}} \\
\cmidrule(lr){4-11}
\cmidrule(lr){12-19}
\cmidrule(l){20-20}
 & \textbf{Strategy} & \textbf{Configuration} & \textbf{Avg} & \textbf{SPAT} & \textbf{TEMP} & \textbf{DETL} & \textbf{EVNT} & \textbf{SOC} & \textbf{CAUS} & \textbf{PROS} & \textbf{Avg} & \textbf{Inst} & \textbf{Short} & \textbf{S-Mid} & \textbf{Mid} & \textbf{ML} & \textbf{Long} & \textbf{Ultra} & \textbf{Proc.} \\
\midrule
\multicolumn{20}{@{}l}{\textit{Sliding-window baselines}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_sw_pura} & \bFIFO & Sliding Window & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{29.53} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.50} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{33.53} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.62} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{30.02} & \cellcolor[HTML]{A2D99C}\textcolor[HTML]{000000}{26.85} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{25.94} & \cellcolor[HTML]{D3EECD}\textcolor[HTML]{000000}{29.28} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{28.33} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{31.83} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{31.09} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{28.71} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.80} & \cellcolor[HTML]{CBEAC4}\textcolor[HTML]{000000}{28.42} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{28.12} & \cellcolor[HTML]{AEDEA7}\textcolor[HTML]{000000}{22.37} & \cellcolor[HTML]{FFF5F0}\textcolor[HTML]{000000}{1.05} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sw_sink} & \bFIFO\ \bSink & StreamVLM~\cite{xu2025streamingvlm} & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{44.74} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{57.95} & \cellcolor[HTML]{248C46}\textcolor[HTML]{FFFFFF}{51.22} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{54.90} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{46.36} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{28.87} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{38.68} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{35.20} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{39.05} & \cellcolor[HTML]{005120}\textcolor[HTML]{FFFFFF}{55.06} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{55.10} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{49.18} & \cellcolor[HTML]{208843}\textcolor[HTML]{FFFFFF}{40.00} & \cellcolor[HTML]{7FC97F}\textcolor[HTML]{000000}{29.34} & \cellcolor[HTML]{46AE60}\textcolor[HTML]{FFFFFF}{24.93} & \cellcolor[HTML]{D3EECD}\textcolor[HTML]{000000}{19.74} & \cellcolor[HTML]{FFF4EF}\textcolor[HTML]{000000}{1.07} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based merge \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_pseudo_att} & \bMerge\ \bIntraPA & CaM-like~\cite{zhang2024cam} & \cellcolor[HTML]{1E8741}\textcolor[HTML]{FFFFFF}{41.87} & \cellcolor[HTML]{17813D}\textcolor[HTML]{FFFFFF}{54.25} & \cellcolor[HTML]{43AC5E}\textcolor[HTML]{FFFFFF}{48.20} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{51.49} & \cellcolor[HTML]{248C46}\textcolor[HTML]{FFFFFF}{42.48} & \cellcolor[HTML]{39A257}\textcolor[HTML]{FFFFFF}{28.27} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{37.48} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{30.92} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{37.73} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{52.47} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{51.98} & \cellcolor[HTML]{3BA458}\textcolor[HTML]{FFFFFF}{44.00} & \cellcolor[HTML]{52B365}\textcolor[HTML]{FFFFFF}{37.20} & \cellcolor[HTML]{BAE3B3}\textcolor[HTML]{000000}{28.65} & \cellcolor[HTML]{86CC85}\textcolor[HTML]{000000}{23.48} & \cellcolor[HTML]{66BD6F}\textcolor[HTML]{000000}{26.32} & \cellcolor[HTML]{FC8B6B}\textcolor[HTML]{000000}{2.87} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_cosine} & \bMerge\ \bIntraCos & CaM-like~\cite{zhang2024cam} & \cellcolor[HTML]{03702E}\textcolor[HTML]{FFFFFF}{43.42} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{57.30} & \cellcolor[HTML]{329B51}\textcolor[HTML]{FFFFFF}{49.83} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{53.28} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{45.87} & \cellcolor[HTML]{72C375}\textcolor[HTML]{000000}{27.52} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{38.53} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{258D47}\textcolor[HTML]{FFFFFF}{38.10} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{54.44} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{53.20} & \cellcolor[HTML]{0C7735}\textcolor[HTML]{FFFFFF}{48.18} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{39.40} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.50} & \cellcolor[HTML]{9CD797}\textcolor[HTML]{000000}{22.90} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{FCB296}\textcolor[HTML]{000000}{2.33} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based hybrid merge + prune \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_merge_intra_pseudo_att_inter_pseudo_att} & \bMerge\ \bIntraPA\ \bPrune\ \bInterPA & -- & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{43.44} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{56.66} & \cellcolor[HTML]{147E3A}\textcolor[HTML]{FFFFFF}{52.62} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{53.89} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{45.33} & \cellcolor[HTML]{CDECC7}\textcolor[HTML]{000000}{26.10} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{38.23} & \cellcolor[HTML]{8ACE88}\textcolor[HTML]{000000}{31.25} & \cellcolor[HTML]{268E47}\textcolor[HTML]{FFFFFF}{38.01} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{54.61} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{52.87} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{47.35} & \cellcolor[HTML]{228A44}\textcolor[HTML]{FFFFFF}{39.87} & \cellcolor[HTML]{A8DCA2}\textcolor[HTML]{000000}{28.88} & \cellcolor[HTML]{CDECC7}\textcolor[HTML]{000000}{21.45} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{8A0812}\textcolor[HTML]{FFFFFF}{5.32} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Similarity-based prune \bFIFO\ \bSink\ \bHat +}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cross_sink} & \bPrune\ \bIntraCS & StreamMem~\cite{yang2025streammem} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{42.39} & \cellcolor[HTML]{29914A}\textcolor[HTML]{FFFFFF}{52.25} & \cellcolor[HTML]{1D8640}\textcolor[HTML]{FFFFFF}{51.80} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{52.10} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{43.85} & \cellcolor[HTML]{87CD86}\textcolor[HTML]{000000}{27.23} & \cellcolor[HTML]{03702E}\textcolor[HTML]{FFFFFF}{37.93} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{38.88} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{52.12} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{50.64} & \cellcolor[HTML]{289049}\textcolor[HTML]{FFFFFF}{45.82} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{39.07} & \cellcolor[HTML]{CBEAC4}\textcolor[HTML]{000000}{28.42} & \cellcolor[HTML]{2D954D}\textcolor[HTML]{FFFFFF}{25.80} & \cellcolor[HTML]{278F48}\textcolor[HTML]{FFFFFF}{30.26} & \cellcolor[HTML]{B01217}\textcolor[HTML]{FFFFFF}{4.91} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm} & \bPrune\ \bIntraVN & InfiniPot-V (VaN)~\cite{kim2025infinipotv} & \cellcolor[HTML]{00692A}\textcolor[HTML]{FFFFFF}{43.79} & \cellcolor[HTML]{0B7734}\textcolor[HTML]{FFFFFF}{55.54} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{53.67} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{52.49} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{45.98} & \cellcolor[HTML]{137D39}\textcolor[HTML]{FFFFFF}{29.02} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{38.23} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{39.17} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{54.30} & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{51.87} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{46.88} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{41.93} & \cellcolor[HTML]{9FD899}\textcolor[HTML]{000000}{29.00} & \cellcolor[HTML]{3CA559}\textcolor[HTML]{FFFFFF}{25.22} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{DC2924}\textcolor[HTML]{FFFFFF}{4.23} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_inter_cosine} & \bPrune\ \bInterCos & InfiniPot-V (TaR)~\cite{kim2025infinipotv} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{45.23} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{57.87} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{53.78} & \cellcolor[HTML]{005120}\textcolor[HTML]{FFFFFF}{55.60} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{45.76} & \cellcolor[HTML]{46AE60}\textcolor[HTML]{FFFFFF}{28.05} & \cellcolor[HTML]{00471C}\textcolor[HTML]{FFFFFF}{39.73} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{35.86} & \cellcolor[HTML]{006529}\textcolor[HTML]{FFFFFF}{40.16} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{54.75} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{52.76} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{48.82} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{43.87} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{26.38} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{23.68} & \cellcolor[HTML]{AB1016}\textcolor[HTML]{FFFFFF}{4.99} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm_inter_cosine} & \bPrune\ \bIntraVN\ \bInterCos & InfiniPot-V~\cite{kim2025infinipotv} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{44.52} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{58.91} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{56.23} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{55.51} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{46.36} & \cellcolor[HTML]{CDECC7}\textcolor[HTML]{000000}{26.10} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{39.58} & \cellcolor[HTML]{DDF2D8}\textcolor[HTML]{000000}{28.95} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{40.22} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{54.44} & \cellcolor[HTML]{005321}\textcolor[HTML]{FFFFFF}{53.93} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{50.12} & \cellcolor[HTML]{006428}\textcolor[HTML]{FFFFFF}{42.27} & \cellcolor[HTML]{268E47}\textcolor[HTML]{FFFFFF}{30.38} & \cellcolor[HTML]{CDECC7}\textcolor[HTML]{000000}{21.45} & \cellcolor[HTML]{37A055}\textcolor[HTML]{FFFFFF}{28.95} & \cellcolor[HTML]{D11E1F}\textcolor[HTML]{FFFFFF}{4.42} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:0_12_q3vl8b_sim_prune_intra_pseudo_att_inter_cosine_octer} & \bPrune\ \bIntraPA\ \bInterCos & StreamTOM~\cite{chen2025streamingtom} w/o \bOff & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{45.19} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{57.87} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{57.28} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.68} & \cellcolor[HTML]{00471C}\textcolor[HTML]{FFFFFF}{46.58} & \cellcolor[HTML]{369F54}\textcolor[HTML]{FFFFFF}{28.35} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{37.78} & \cellcolor[HTML]{72C375}\textcolor[HTML]{000000}{31.79} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{40.43} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{55.42} & \cellcolor[HTML]{004D1F}\textcolor[HTML]{FFFFFF}{54.37} & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{50.88} & \cellcolor[HTML]{016E2D}\textcolor[HTML]{FFFFFF}{41.73} & \cellcolor[HTML]{006027}\textcolor[HTML]{FFFFFF}{31.07} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{25.88} & \cellcolor[HTML]{98D594}\textcolor[HTML]{000000}{23.68} & \cellcolor[HTML]{77040F}\textcolor[HTML]{FFFFFF}{5.51} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cosine} & \bPrune\ \bIntraCos & -- & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{45.63} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{60.51} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{52.39} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.61} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{46.64} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{28.50} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{39.88} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{34.87} & \cellcolor[HTML]{0B7734}\textcolor[HTML]{FFFFFF}{39.34} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{55.60} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{54.99} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{52.18} & \cellcolor[HTML]{0A7633}\textcolor[HTML]{FFFFFF}{41.27} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{30.61} & \cellcolor[HTML]{46AE60}\textcolor[HTML]{FFFFFF}{24.93} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{15.79} & \cellcolor[HTML]{FCB69B}\textcolor[HTML]{000000}{2.28} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_pseudo_att} & \bPrune\ \bIntraPA & -- & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{45.12} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{59.47} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{53.08} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{56.52} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{45.87} & \cellcolor[HTML]{238B45}\textcolor[HTML]{FFFFFF}{28.72} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{39.28} & \cellcolor[HTML]{3EA75A}\textcolor[HTML]{FFFFFF}{32.89} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{41.50} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{56.04} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{54.71} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{50.18} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{40.60} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{A8DCA2}\textcolor[HTML]{000000}{22.61} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{35.53} & \cellcolor[HTML]{FC8F6F}\textcolor[HTML]{000000}{2.82} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_inter_pseudo_attn} & \bPrune\ \bInterPA & -- & \cellcolor[HTML]{00481D}\textcolor[HTML]{FFFFFF}{45.42} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{59.87} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{55.53} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{56.17} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{45.65} & \cellcolor[HTML]{81CA81}\textcolor[HTML]{000000}{27.30} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{38.53} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{34.87} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{40.30} & \cellcolor[HTML]{004C1E}\textcolor[HTML]{FFFFFF}{55.42} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{54.32} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{49.35} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{42.80} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{30.84} & \cellcolor[HTML]{60BA6C}\textcolor[HTML]{FFFFFF}{24.35} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{B61319}\textcolor[HTML]{FFFFFF}{4.82} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_pseudo_att_inter_pseudo_att} & \bPrune\ \bIntraPA\ \bInterPA & -- & \cellcolor[HTML]{005622}\textcolor[HTML]{FFFFFF}{44.71} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{58.51} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{55.30} & \cellcolor[HTML]{00451C}\textcolor[HTML]{FFFFFF}{56.52} & \cellcolor[HTML]{005B25}\textcolor[HTML]{FFFFFF}{45.54} & \cellcolor[HTML]{2B934B}\textcolor[HTML]{FFFFFF}{28.57} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{39.58} & \cellcolor[HTML]{DDF2D8}\textcolor[HTML]{000000}{28.95} & \cellcolor[HTML]{00682A}\textcolor[HTML]{FFFFFF}{40.03} & \cellcolor[HTML]{004A1E}\textcolor[HTML]{FFFFFF}{55.55} & \cellcolor[HTML]{005522}\textcolor[HTML]{FFFFFF}{53.87} & \cellcolor[HTML]{005E26}\textcolor[HTML]{FFFFFF}{50.29} & \cellcolor[HTML]{00692A}\textcolor[HTML]{FFFFFF}{42.00} & \cellcolor[HTML]{75C477}\textcolor[HTML]{000000}{29.46} & \cellcolor[HTML]{137D39}\textcolor[HTML]{FFFFFF}{26.67} & \cellcolor[HTML]{AEDEA7}\textcolor[HTML]{000000}{22.37} & \cellcolor[HTML]{67000D}\textcolor[HTML]{FFFFFF}{5.66} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_vnorm_inter_pseudo_att} & \bPrune\ \bIntraVN\ \bInterPA & -- & \cellcolor[HTML]{005C25}\textcolor[HTML]{FFFFFF}{44.42} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{57.62} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{56.46} & \cellcolor[HTML]{00491D}\textcolor[HTML]{FFFFFF}{56.21} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{46.75} & \cellcolor[HTML]{A2D99C}\textcolor[HTML]{000000}{26.85} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{39.43} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{27.63} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{39.91} & \cellcolor[HTML]{005020}\textcolor[HTML]{FFFFFF}{55.10} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{54.04} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{50.06} & \cellcolor[HTML]{006729}\textcolor[HTML]{FFFFFF}{42.13} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{30.15} & \cellcolor[HTML]{9CD797}\textcolor[HTML]{000000}{22.90} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{C1161B}\textcolor[HTML]{FFFFFF}{4.67} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_cross_sink_inter_pseudo_att} & \bPrune\ \bIntraCS\ \bInterPA & -- & \cellcolor[HTML]{005C25}\textcolor[HTML]{FFFFFF}{44.39} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{56.74} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{52.50} & \cellcolor[HTML]{005221}\textcolor[HTML]{FFFFFF}{55.56} & \cellcolor[HTML]{006227}\textcolor[HTML]{FFFFFF}{45.22} & \cellcolor[HTML]{17813D}\textcolor[HTML]{FFFFFF}{28.95} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{39.88} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{31.91} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{39.60} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{55.24} & \cellcolor[HTML]{004D1F}\textcolor[HTML]{FFFFFF}{54.43} & \cellcolor[HTML]{0D7836}\textcolor[HTML]{FFFFFF}{48.12} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{40.60} & \cellcolor[HTML]{3CA559}\textcolor[HTML]{FFFFFF}{30.03} & \cellcolor[HTML]{7AC77B}\textcolor[HTML]{000000}{23.77} & \cellcolor[HTML]{80CA80}\textcolor[HTML]{000000}{25.00} & \cellcolor[HTML]{B31218}\textcolor[HTML]{FFFFFF}{4.87} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Offloading-based memory management \bFIFO \bSink\ \bHat}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_rekv_offloading} & \bOff & ReKV~\cite{di2025rekv} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{40.99} & \cellcolor[HTML]{2E964D}\textcolor[HTML]{FFFFFF}{51.69} & \cellcolor[HTML]{369F54}\textcolor[HTML]{FFFFFF}{49.48} & \cellcolor[HTML]{2E964D}\textcolor[HTML]{FFFFFF}{48.99} & \cellcolor[HTML]{1E8741}\textcolor[HTML]{FFFFFF}{42.86} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{29.99} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{35.98} & \cellcolor[HTML]{F1FAEE}\textcolor[HTML]{000000}{27.96} & \cellcolor[HTML]{3CA559}\textcolor[HTML]{FFFFFF}{36.83} & \cellcolor[HTML]{137D39}\textcolor[HTML]{FFFFFF}{51.36} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{47.97} & \cellcolor[HTML]{3BA458}\textcolor[HTML]{FFFFFF}{44.00} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{38.67} & \cellcolor[HTML]{8ACE88}\textcolor[HTML]{000000}{29.23} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{25.51} & \cellcolor[HTML]{C2E7BB}\textcolor[HTML]{000000}{21.05} & \cellcolor[HTML]{FDC6B0}\textcolor[HTML]{000000}{2.03} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_rekv_offloading_8bit} & \bQOff & ReKV~\cite{di2025rekv} w/ \bQOff & \cellcolor[HTML]{228A44}\textcolor[HTML]{FFFFFF}{41.63} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{51.85} & \cellcolor[HTML]{2A924A}\textcolor[HTML]{FFFFFF}{50.64} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{50.83} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{43.63} & \cellcolor[HTML]{72C375}\textcolor[HTML]{000000}{27.52} & \cellcolor[HTML]{349D53}\textcolor[HTML]{FFFFFF}{35.38} & \cellcolor[HTML]{7CC87C}\textcolor[HTML]{000000}{31.58} & \cellcolor[HTML]{17813D}\textcolor[HTML]{FFFFFF}{38.77} & \cellcolor[HTML]{05712F}\textcolor[HTML]{FFFFFF}{52.61} & \cellcolor[HTML]{309950}\textcolor[HTML]{FFFFFF}{47.74} & \cellcolor[HTML]{45AD5F}\textcolor[HTML]{FFFFFF}{43.12} & \cellcolor[HTML]{2C944C}\textcolor[HTML]{FFFFFF}{39.27} & \cellcolor[HTML]{0E7936}\textcolor[HTML]{FFFFFF}{30.72} & \cellcolor[HTML]{1C8540}\textcolor[HTML]{FFFFFF}{26.38} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{31.58} & \cellcolor[HTML]{FEE2D5}\textcolor[HTML]{000000}{1.59} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Other}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_sim_prune_intra_pseudo_att_inter_cosine_no_hat} & Q3VL8B_sim_prune_intra_pseudo_att_inter_cosine_no_hat & -- & \cellcolor[HTML]{005C25}\textcolor[HTML]{FFFFFF}{44.38} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{58.75} & \cellcolor[HTML]{006D2C}\textcolor[HTML]{FFFFFF}{54.25} & \cellcolor[HTML]{00471C}\textcolor[HTML]{FFFFFF}{56.39} & \cellcolor[HTML]{005120}\textcolor[HTML]{FFFFFF}{46.04} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{24.98} & \cellcolor[HTML]{005924}\textcolor[HTML]{FFFFFF}{38.98} & \cellcolor[HTML]{8ACE88}\textcolor[HTML]{000000}{31.25} & \cellcolor[HTML]{006328}\textcolor[HTML]{FFFFFF}{40.23} & \cellcolor[HTML]{004E1F}\textcolor[HTML]{FFFFFF}{55.28} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{53.09} & \cellcolor[HTML]{067230}\textcolor[HTML]{FFFFFF}{48.76} & \cellcolor[HTML]{006428}\textcolor[HTML]{FFFFFF}{42.27} & \cellcolor[HTML]{005723}\textcolor[HTML]{FFFFFF}{31.19} & \cellcolor[HTML]{F7FCF5}\textcolor[HTML]{000000}{19.42} & \cellcolor[HTML]{157F3B}\textcolor[HTML]{FFFFFF}{31.58} & \cellcolor[HTML]{B91419}\textcolor[HTML]{FFFFFF}{4.76} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Offloading-based memory management \bFIFO \bSink\ \bHat}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:streamtom_like} & \bPrune\ \bIntraPA\ \bInterCos\ \bQOff - \bHat & StreamingTOM~\cite{chen2025streamingtom} & \cellcolor[HTML]{0C7735}\textcolor[HTML]{FFFFFF}{42.86} & \cellcolor[HTML]{1D8640}\textcolor[HTML]{FFFFFF}{53.61} & \cellcolor[HTML]{16803C}\textcolor[HTML]{FFFFFF}{52.39} & \cellcolor[HTML]{117B38}\textcolor[HTML]{FFFFFF}{51.88} & \cellcolor[HTML]{026F2E}\textcolor[HTML]{FFFFFF}{44.51} & \cellcolor[HTML]{4DB163}\textcolor[HTML]{FFFFFF}{27.97} & \cellcolor[HTML]{077331}\textcolor[HTML]{FFFFFF}{37.78} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{31.91} & \cellcolor[HTML]{006B2B}\textcolor[HTML]{FFFFFF}{39.93} & \cellcolor[HTML]{005F26}\textcolor[HTML]{FFFFFF}{54.03} & \cellcolor[HTML]{278F48}\textcolor[HTML]{FFFFFF}{48.69} & \cellcolor[HTML]{2F984F}\textcolor[HTML]{FFFFFF}{45.06} & \cellcolor[HTML]{208843}\textcolor[HTML]{FFFFFF}{40.00} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{31.42} & \cellcolor[HTML]{258D47}\textcolor[HTML]{FFFFFF}{26.09} & \cellcolor[HTML]{005A24}\textcolor[HTML]{FFFFFF}{34.21} & \cellcolor[HTML]{FEE7DC}\textcolor[HTML]{000000}{1.43} \\

\midrule
\multicolumn{20}{@{}l}{\textit{Other}} \\

\refstepcounter{rowcount}\arabic{rowcount}\label{row:q3vl8b_rekv_offloading_no_sink} & Q3VL8B_rekv_offloading_no_sink & -- & \cellcolor[HTML]{3FA95C}\textcolor[HTML]{FFFFFF}{39.68} & \cellcolor[HTML]{53B466}\textcolor[HTML]{FFFFFF}{47.91} & \cellcolor[HTML]{2B934B}\textcolor[HTML]{FFFFFF}{50.52} & \cellcolor[HTML]{46AE60}\textcolor[HTML]{FFFFFF}{46.54} & \cellcolor[HTML]{2F974E}\textcolor[HTML]{FFFFFF}{41.77} & \cellcolor[HTML]{39A257}\textcolor[HTML]{FFFFFF}{28.27} & \cellcolor[HTML]{76C578}\textcolor[HTML]{000000}{32.83} & \cellcolor[HTML]{BEE5B8}\textcolor[HTML]{000000}{29.93} & \cellcolor[HTML]{48AE60}\textcolor[HTML]{FFFFFF}{36.34} & \cellcolor[HTML]{359E53}\textcolor[HTML]{FFFFFF}{48.11} & \cellcolor[HTML]{6BC072}\textcolor[HTML]{000000}{43.57} & \cellcolor[HTML]{52B365}\textcolor[HTML]{FFFFFF}{42.41} & \cellcolor[HTML]{2F984F}\textcolor[HTML]{FFFFFF}{39.00} & \cellcolor[HTML]{1F8742}\textcolor[HTML]{FFFFFF}{30.49} & \cellcolor[HTML]{00441B}\textcolor[HTML]{FFFFFF}{28.41} & \cellcolor[HTML]{AEDEA7}\textcolor[HTML]{000000}{22.37} & \cellcolor[HTML]{FDCCB8}\textcolor[HTML]{000000}{1.94} \\

\bottomrule
\end{tabular}%
}
\end{table}
